BClean: A Bayesian Data Cleaning System

There is a considerable body of work on data cleaning which employs various principles to rectify erroneous data and transform a dirty dataset into a cleaner one. One of prevalent approaches is probabilistic methods, including Bayesian methods. However, existing probabilistic methods often assume a simplistic distribution (e.g., Gaussian distribution), which is frequently underfitted in practice, or they necessitate experts to provide a complex prior distribution (e.g., via a programming language). This requirement is both labor-intensive and costly, rendering these methods less suitable for real-world applications. In this paper, we propose BClean, a Bayesian Cleaning system that features automatic Bayesian network construction and user interaction. We recast the data cleaning problem as a Bayesian inference that fully exploits the relationships between attributes in the observed dataset and any prior information provided by users. To this end, we present an automatic Bayesian network construction method that extends a structure learning-based functional dependency discovery method with similarity functions to capture the relationships between attributes. Furthermore, our system allows users to modify the generated Bayesian network in order to specify prior information or correct inaccuracies identified by the automatic generation process. We also design an effective scoring model (called the compensative scoring model) necessary for the Bayesian inference. To enhance the efficiency of data cleaning, we propose several approximation strategies for the Bayesian inference, including graph partitioning, domain pruning, and pre-detection. By evaluating on both real-world and synthetic datasets, we demonstrate that BClean is capable of achieving an F-measure of up to 0.9 in data cleaning, outperforming existing Bayesian methods by 2% and other data cleaning methods by 15%.

==> background.tex <==
\section{Preliminary}

\subsection{Bayesian Network}
Bayesian Network is known as a belief network, is an extension of Bayesian
method and is currently one of the most effective theoretical models in the
field of uncertain knowledge expression and reasoning. The definition of
probability distribution $p(x|D)$ is as follows.
\begin{equation}
    \centering
    P(X_{1},X_{2},...,X_{n}) = \prod \limits_{i} P(X_{i}|Par_{G}(X_{i}))
\end{equation}
\qquad Where $Par_{G}(X_{i})$ represents the parents' node which have impact on the
current node. Bayesian Network is a directed acyclic graph. Given some observed
variable, hidden variable can be computed. And finally the whole network
structure that conditional probability distribution $p(x|D)$ is inferred, where
x is current node and D is the observed variable.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> definition-yukai.tex <==
\section{Definitions and Framework}

We formally provide the problem definitions first, followed by an overview of
\bclean's solution to data clean.

\subsection{Problem Definition} 
The goal of \bclean is to repair a structured dataset $D$ with a Bayesian
Network(BN). Finally return a cleaner version of $D$ by repairing the erroneous
data. We denote $n$ tuples of observations as $D_{obs}=\{T_{0}, T_{1}, ...,
T_{n}\}$ and $m$ attributes as $A=\{A_{0}, A_{1}, ..., A_{m}\}$. Let $G=\{G_{0},
G_{1}, ..., G_{n}\}$ be a repair, in which $G_{i}=\{A_{0}^{*}, A_{1}^{*}, ...,
A_{m}^{*}\}$ is the clean version of the $i^{th}$ tuple
% be a repair candidate of the $i^{th}$ tuple
. To clean $T_{i}$, BClean aims to infer the most likely $g$ in $G_{i}$, where
$g\in dom(A_{i})$ is the candidate of a specific cell $T_i[A_j]$ and $dom(A_{i})$
is the domain of attribute $A_{i} \in A$. If $T_{i}$ is clean, $G_{i}=T_{i}$
will hold. In general, we denote the task as finding the $G_{i} \in
G$ with the highest probability under the constraints of user's requirement.
% Bayesian Network as $Pr[D]$ expressed as probabilistic model and score-based association model $Prior\_Score$ expressed as transformed probabilistic model. 
Formally, we define the probabilistic inference problem as follow:
\begin{equation}
    G^{*} = \arg \max \prod_{G_{i} \in G} Pr[G_{i}] \quad subject \ to \ User(G_{i})
\end{equation}

% User（G{i}）定义
Where $User(G_{i})$ is denoted as constraints encoded by user requirements and is XX to set value that meet the requirements to Null. Formally.
\begin{equation}
    User(G_{i})=
\end{equation}
%User（G{i}）定义
In practice, 
% errors in $D_{obs}$ occur due to aforementioned users' carelessly input, system's bug
% or some insufficient support from hardware. 
We repair the errors by updating
the values of $T_{i}[A_{j}]$ in $D_{obs}$ if $T_{i}[A_{j}]$ is dirty. In $T_{i}[A_{j}]$, We denote $v_{obs}$ the observation and $v_{clean}$ the unknown ground-truth. We define $T_{i}[A_{j}]$ a error cell for 
satisfying $v_{obs}\ne v_{clean}$. To repair $D_{obs}$, BClean infers
the latent true value $v_{infer}$ given the relevant $\{T_{i}[A_{k}]|k \neq j\}$ from $D_{obs}$. As for inferred value $v_{infer}$, we
say that the cell is clean because of $v_{infer}=v_{clean}\land
v_{infer}=v_{obs}$. And if $v_{infer}=v_{clean}\land v_{infer}\ne v_{obs}$, we
determine that the cell is dirty and $v_{infer}$ will replace the $v_{obs}$ as
repair. In general, we combine error detection and repair into one system.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Images/BN skeleton2.png}
    \caption{Bayesian Network Skeleton learn from real-world datase}
    \label{BNskeleton}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{Images/overview.png}
    \caption{An overview of BClean framework for data clean}
    \label{Overview}
\end{figure*}

\noindent\textbf{Preliminary.}
The Bayesian Network , known as a belief network, is an extension of Bayesian
method and is currently one of the most effective theoretical models in the
field of uncertain knowledge expression and
inference \cite{DBLP:journals/ker/Parsons11a}. The Bayesian network is a Directed
Acyclic Graph (DAG) $(N,E,\theta)$, which is composed of a set of nodes ${N}$
representing variables ,a set of directed edges ${E}$ connecting these nodes and
a set of Conditional Probabilistic Table(CPT) $\theta$ weighting $E$. Nodes
represent random variables, and the directed edges between nodes represent the
casual relationship between nodes (from the parent node to its child nodes).
Conditional probability $\theta$ is used to express the strength of the causality. If there is no parent node, the prior probability is expressed by
prior information. Bayesian Network can be expressed as a probability
distribution $Pr(X_{i})$, where $X_{i} \in N$. And the definition of
$Pr(X_{i})$ is formulized as follows,
\begin{equation}
    \centering
    Pr(X_{1},X_{2},...,X_{n}) = \prod \limits_{X_{i} \in N} Pr(X_{i}|Par_{G}(X_{i}))
\end{equation}

Where $Par_{G}(X_{i})$ represents the parents' node which have impact on
the current node. For those nodes without parents, the information of
$Par_{G}(X_{i})$ is provided by prior. Given some observed variable, hidden
variable can be computed. And finally the whole network structure that
conditional probability distribution $p(x|D)$ is inferred, where x is current
node and D is the observed variable. In fact, different structure learning
algorithm generate diverse skeletons with similar causality. Figure
\ref{BNskeleton} show a Bayesian Network skeleton learning from real-world
dataset.


We found that $State="CA"$ and $InsuranceType="Normal"$ can be firmly calculated
in line 1 and 2 of Table \ref{ExampleDataset}. If $Jobid$ is wrong in line 2,
$Name$ and $Department$ won't be independent according to Bayesian Network's
definition. And with users help to match or filter some candidates, we can get
one candidate repair $Department="315\ w\ hickory\ st"$ due to $Name="Jonny.R"$
in BN. And $Jobid="25676000"$ in line 2 is also available. In line 4-6,
$Department$ is completely wrong but without label. However, we still can
rank the domain as candidate set. And we also ask user for help about other
cell in the same tuple for information's confidence. It can help judge that line
5 is unreliable about its correlation. Thus for line 4-6, we get final repair
$Department="400\ northwood\ dr"$, $State="KT"$, $ZipCode="35960"$,
$InsuranceCode="2560018035960" (Jobid, ZipCode \rightarrow InsuranceCode)$ and
$InsuranceType="Low"$ due to our approach's getting rid of the relationship from
line 5.


\subsection{Solution Overview}
An overview of BClean is shown in Figure \ref{Overview}. BClean takes as input a
dataset D as observation along with parameters offered by users. The parameters
is designed as defining a schema and only requires, maximum and
minimal length(value), Null permitted or not, repair-need or not, values pattern
and even some fix casualty within attributes from observation, which even are
optional(e.g, users is allowed to offer a incomplete set of parameters if they
can't firmly depict it like defining a relation schema.). BClean’s workflow
follows two steps:

\noindent\textbf{Probabilistic Modeling.}
The first step is to generate BN and collect the dictionary of frequency and co-occurrence about observation with users' providing information. Besides existing BN structure learning based on
constraints, score and hybrid algorithm
such as PC, HillClimbSearch based on different score method and
MMHC\cite{DBLP:journals/ml/TsamardinosBA06}that have been developed in toolkit
Pgmpy\cite{ankan2015pgmpy}(i.e. different structure algorithm generates
different BN with similar casualty), we try to use the structure method based on Grapical Lasso~\cite{DBLP:conf/nips/WuSD19} and a directed graph structure learning method~\cite{raskutti2018learning}.
% And then shown the skeleton DAG to user.
% Users can pick one that is considered to be the most reasonable. 
In processing
of generating Association Model, we collect all observation for each attribute as its frequency of domain and 
 and pairwise attributes correlation.

\noindent\textbf{Inference Grounding with Pruning.}In this step, we have already get
a BN with CPT learning from $D_{obs}$ and a Association Model collecting frequency.
% every tuple about the correlation dictionary in last step. 
In this step, we propose a way to measure how correct $v \in dom(A_{j})$ is with BN and Association Model. For every $v \in dom(A_{j})$, the probability of clean is calculated. However, there exists unnecessary calculation in reference. Thus, We pruned the calculation from three aspects.(i) According to Markov property~\cite{DBLP:journals/ker/Parsons11a}, we make partitional inference on Bayesian network, which reduces the cost of variable elimination.(ii) Based on the semantics of partitional network, we prune the domain and discard the values that obviously do not conform to the semantics.(iii)We use Association Model to propose a pre-detection, and propose inference for some variable that are probably correct.
% the most
% significant operation is the consideration about whether the correlation in a
% specific tuple is reliable and its probability when holds. 
% Thus we set a \emph{Confidence} to measure the
% reliability. For example, in line 5 of Table \ref{ExampleDataset}, we found that
% value of cell $Department$, $ZipCode$, $InsuranceCode$ is apparently wrong by
% user's pre-definition. And its \emph{Confidence} is lower than threshold also
% defined by user. Therefore, we view relationship shown in line 5 as unreliable
% and set penalty to it.


% \noindent\textbf{Grounding Pruning.}
% In this step, we focus on reducing unnecessarily calculation in inference. We pruned the calculation from three aspects.(i) According to Markov property~\cite{DBLP:journals/ker/Parsons11a}, we make partitional inference on Bayesian network, which reduces the cost of variable elimination.(ii) Based on the semantics of partitional network, we prune the domain and discard the values that obviously do not conform to the semantics.(iii)We use Association Model to propose a pre-detection, and propose inference for some variable that are probably correct.
% have already get the whole conditional probabilistic
% distribution and relation pairwise except in BN model. We combine the prior
% model and BN model. For each attribute, We denote the values of domains the
% candidate set of attributes. And then we run BN model to compute every
% candidate. Finally we pick up the best candidate to act as $v_{infer}$ with
% highest score computed by BN under the constraints of association model.


==> response.tex <==

%\author{\vspace{-3ex}}
%\date{Feburary 16, 2013}

\renewcommand{\reviseX}[1]{{\color{black}{#1}}}
\renewcommand{\irevise}[1]{{\color{black}{#1}}}
%\renewcommand{\warnr}[1]{{\color{black}{#1}}}
%\renewcommand{\warnX}[1]{{\color{black}{#1}}}


\twocolumn
\balance

\section*{Paper 503: Response to Reviews}
\vspace{2ex}

% \noindent
% Dear Referees and Meta Reviewer:

% \vspace{0.8ex}
% The paper has been substantially revised. We have addressed all the
% issues raised in the reviews and meta review.
% %according to the referees' comments
% %and the meta review. In particular, we have ... in response to Meta-Review. 

We appreciate the meta-reviewer and the reviewers' comments and suggestions that 
help us to improve the paper. We revised the paper according to the 
requested changes.  
% For the convenience of Referees, changes to the paper 
% are color-coded in \revise{\color{blue}{blue}}.
%, in response to the suggestions of Referees~1, 2, 3 and~4, respectively.
Major changes in the revised paper are marked in \revise{blue}. 
Next, we provide our responses to the comments. 
References to the revised paper are marked in \reviseR{red}. 

% We would like to thank all the referees
% for their thorough reading of our paper
% and for their helpful comments.

%Below please find our responses to the comments by the referees.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{2ex}
% \hrule
% \vspace{0.6ex}
% \ni
% {\bf Response to the comments of Meta Review.}
% \vs


% \ni
% {\em
% 	{\bf [Required Changes]} All revision items listed in Field 13 of the reviews. In particular:

% \vspace{-1ex}
% \stab
% 	 (a). R1: O1, O2, O3

% \vspace{-1ex}
% \stab
% 	 (b). R2: O1, O2, O3, O4, O5, O6, O7

% \vspace{-1ex}
% \stab
% 	 (c). R5: O1, O2, O3, O4
% }



% \vs
% \ni
%    {\bf [A]}
%  Thanks! We have supplemented detailed explanations and new experiments.

% \vspace{1.8ex}
% \ni
% {\em
% 	{\bf [Optional Changes]}
% R5: O2, O3
% }

% \vs
% \ni
% {\bf [A]}
% \reviseT{We have also addressed %these related to
% O2 and O3 of R5. 
% }

% %\vspace{2ex}
% %We thank for supporting this work!
% %the positive feedback!

% \ni
% Meta-reviewer's comments correspond to (must-revise):

% \begin{itemize}
%   \item R1.O1, O2.
%   \item R2.O2.2, O2.3.
%   \item R1.O3.
%   \item R3.O2(one dimension), additional remarks.
%   \item R3.O2(third).
%   \item R3.additional remarks.
% \end{itemize}

% \wys{Unsolved Question in draft: R1-O2, R1-D2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{3ex}
\hrule
\vspace{0.6ex}
\ni
{\bf Response to the comments of Reviewer \#1.}
\vs

\ni
{\em
{\bf [O1]}
Easy-to-deploy data cleaning. 
}

\ni
{\bf [A]}
We modified the introduction (\reviseR{Section \ref{sec:intro}}) to explain 
\bclean's easy-to-deploy data cleaning. We also provide the details of the UCs 
used in this paper (\reviseR{Section \ref{sec:preliminaries}}). 

In general, existing solutions (e.g., \pclean, \raha) need to inject prior 
distributions or error distributions of attributes, ground truth labeling, denial 
constraints (DCs), or programs in probabilistic programming language (PPL), which 
are often not easy to obtain or require professional skills which are  
% Some example PPL programs can be found in Appendix B.4 of \cite{DBLP:conf/aistats/LewASM21} 
% (e.g., 51 lines of code for the \hospital dataset). 
additional to common data management skills (e.g., SQL, regular expressions). 
In contrast, it is easier for users to accept user constraints (UCs) in \bclean, 
which are simple (e.g., min/max constraints for numerical values, not NULL, regular 
expressions) but effective. 

% We use the following simple but effective UCs in our experiments: 
% \begin{inparaenum} [(1)]
%   \item minimum and maximum value constraints for numerical attributes, 
%   \item not NULL constraints, and 
%   \item simple regular expressions for digits (e.g., Zipcode), dates (e.g., sch\_arr in Flights), and year (e.g., birthyear). 
% \end{inparaenum}

\vs

\ni
{\em
{\bf [O2]} Novelty of the cleaning strategy.
}

\ni   
{\bf [A]}
\vs
% The novelty of \bclean includes:
% \begin{inparaenum} [(1)]
%   \item a Bayesian network (BN) construction based on automatic FD discovery, 
%   \item a compensative scoring model that naturally embeds user constraints that implicitly guide Bayesian inference to correct errors, and 
%   \item approximate inference strategies to accelerate the process without sacrificing much performance. 
% \end{inparaenum}
% Specifically, \bclean differs from existing solutions (\holoclean, \pclean, \raha, etc.) in the following aspects:
% \begin{itemize}
%   \item In \holoclean, factor graphs act as a feature generator to generate the degree of validity 
%   (i.e., feature) for each denial constraint (DC), while \bclean is totally based on a BN, i.e., 
%   it corrects errors entirely with Bayesian inference. 
%   \item Although DCs in \holoclean could be discovered, the errors would be amplified in dirty data. 
%   \bclean is robust and insensitive to dirty data due to the Bayesian inference and the compensative 
%   scoring model. This is demonstrated in the experiments. especially in the additional experiments 
%   added in this revision. 
%   \item \pclean is based on Bayesian inference but its network construction and prior distributions 
%   are hand-crafted, and users have to learn PPL to specify them. In contrast, \bclean is automatic 
%   and only a few simple UCs are needed. 
%   \item \raha + \baran are ML models with automatically generated features as inputs, but they need a 
%   few ground truths to train, while \bclean is unsupervised.
% \end{itemize}
We modified \reviseR{Section \ref{sec:intro}} to highlight the novelty of \bclean. 

\ni
{\em
{\bf [O3]} More details of experiment setup. 
}

\ni   
{\bf [A]}
We modified Section~\ref{sec:exp-setup} to clarify the setup. 
Moreover, the ``patterns'' mentioned in the experiments are regular expressions, e.g., Zipcode 
(\texttt{$\wedge$([1-9][0-9]\{4,4\})\$}) and PhoneNumber (\texttt{$\wedge$([1-9][0-9]\{9,9\})\$}). 
To the best of our knowledge, although DCs support regular expressions 
by adding them as predicates, they are hard to discover or write by hand.
% 1. For \soccer, we randomly inject noises by 
% \begin{inparaenum} [(1)]
%   \item replacing cells with a null value, 
%   \item modifying cells with insertion, deletion, and replacement of characters, and 
%   \item swapping the cell values.
% \end{inparaenum}

% 2. For the UCs used in this paper, please refer to \reviseR{Section \ref{sec:preliminaries}}. 
% For \hospital and \flights, \holoclean used the DCs provided by the authors. For \soccer, DCs 
% are carefully hand-crafted by us. \bclean automatically discovers such rules when the BN is 
% constructed.

% 3. The patterns used in the experiments are regular expressions, e.g., Zipcode 
% (\texttt{$\wedge$([1-9][0-9]{4,4})\$}) and PhoneNumber (\texttt{$\wedge$([1-9][0-9]{9,9})\$}). To the best of our 
% knowledge, although DCs support regular expressions by adding them as predicates, they are 
% hard to discover or write by hand.

%In this revision, we clarified the above settings in \reviseR{Section \ref{sec:exp-setup}}.

\vs

\ni
{\em
{\bf [D2]} Logarithmic forms in Section~\ref{sec:association}. 
}

\ni   
{\bf [A]}
The logarithm form first appears in \reviseR{Section~\ref{sec:model} (Equation~\ref{eq:TransformMultiToAdd})}. 
We added an discussion in \reviseR{Section~\ref{sec:association}} for 
the approximation in the compensative score computation (\reviseR{Equation~\ref{eq:association-appr}}). 
\vs

\ni
{\em
{\bf [D5]} Deep error analysis on the experimental datasets.
}

\ni   
{\bf [A]}
We revised the experiments by adding more datasets and more complex errors. 
Please refer to \reviseR{Section \ref{sec:exp-error-analysis}} for the new 
materials. 
\vs

\ni
{\em
{\bf [D6]} \rahaBaran{}'s user time.
}

\vs
\ni
{\bf [A]}
Labeling is considered as user time for \rahaBaran (\reviseR{Section~\ref{sec:exp-runtime-analysis}}). 

\vspace{3ex}
\hrule
\vspace{0.6ex}
\ni
{\bf Response to the comments of Reviewer \#2.}

%We have made the following revisions as suggested.

%\vspace{1.8ex}
\ni
{\em
{\bf [O2]}
Robustness against change of error rate. 
}

\ni
{\bf [A]}
We added an experiment for varying error rate. Please refer to 
\reviseR{Section \ref{sec:exp-error-analysis} -- Varying error ratio}.
\vs

\ni
{\em
{\bf [O3]}
ML pipelines, type of errors, and FDs.
}

\ni
{\bf [A]}
1. We surveyed related studies (\reviseR{Section \ref{sec:related}}) on the impact 
of data cleaning in ML pipelines. In \cite{cleanml}, there are five types of errors: 
missing values, inconsistencies, outliers, duplicates, mislabels. We focus on the 
first two types of errors in this paper, as outliers and duplicates can be fixed 
by outlier detection/removal and deduplication tools, and mislabels are not applicable 
here since we target data cleaning itself rather than downstream ML tasks. 

\ni
2. We conducted experiments on more datasets as well as more complex errors (as also 
requested by Reviewer \#3). Please refer to the response to Reviewer \#3.O2 for the 
dataset and error settings. 

\ni
3. For FDs, we agree that exact FDs are rarely completely satisfied by the data. Here, 
we adopt two ways to alleviate it: First, we do not directly discover FDs but adopt 
the graphical lasso to generate the inverse covariance matrix, and all we need is the 
matrix to construct a BN. Second, we extend exact FDs to ``soft'' FDs with similarity 
functions. Such discussion appears in the beginning of \reviseR{Section \ref{sec:bn-skeleton}}.
\vs

\ni
{\em
{\bf [O4]}
More discussions on related work.
}

\ni
{\bf [A]}
We modified \reviseR{Section \ref{sec:related}} for more related work and 
discussions. 
%\vs

\vspace{3ex}
\hrule
\vspace{0.6ex}
\ni
{\bf Response to the comments of Reviewer \#3.}
\vs

\ni
{\em
{\bf [O1]}
More details of user constraints (UCs) and experiment setup. 
}

\ni
{\bf [A]}
% As discussed in the response to {\bf[O1]} of Reviewer \#1, the UCs 
% in \bclean are (1) minimum and maximum value constraints for numerical
% attributes, (2) not NULL constraints, and (3) simple regular expressions.
% These UCs require much less expertise from the users than the prior
% distributions or PPL in the baseline methods. 
% In terms of the experiment setup, we trained some undergraduate students to
% use the baseline methods and our \bclean system, and assigned one student to
% each of these methods for the experiment. The UCs deployed in \bclean in the
% experiments are listed in Table~\ref{DatasetSummary}. The time for training
% the users is not included in the reported ``user time''.
We revised \reviseR{Section \ref{sec:preliminaries}} for a clear definition of 
UCs, and also revised \reviseR{Section~\ref{sec:exp-setup}} to provide more 
details of the experiment setup.
We add an user study in \reviseR{Section~\ref{sec:user-study}.}
For PPL program examples, please refer to Appendix B.4 of 
\cite{DBLP:conf/aistats/LewASM21}. We choose not to include them (e.g., 51 lines 
for \hospital) in our paper due to the page limitation. 

\vs

\ni
{\em
{\bf [O2]}
More experiments (datasets, numericals, and complex errors)
}

\ni
{\bf [A]}
1. We added three new datasets, \beers, \inpatient, and \facilities, 
which are described in \reviseR{Section~\ref{sec:exp-setup}}.
%\fixme{introduce the properties of the new datasets and how
%they are made}.

\ni
2. We sampled 50,000 tuples from \soccer and compared \bclean with 
other approaches. The results are shown in \reviseR{Table~\ref{fig:holoclean-soccer}}.
%\fixme{Complete this}

\ni
3. We introduced the technique of handling numerical data in 
\reviseR{Section \ref{sec:numerical}}. For evaluation, we added two 
datasets, \beers and \rents. The results are shown in \reviseR{Tables~\ref{BaselineResult} 
and \ref{fig:msee}}, and the discussions are in \reviseR{Section~\ref{sec:exp-cleanquality}
and \ref{sec:exp-error-analysis}}.

\ni
4. We added \bcleannouc, \bclean without UCs, and reported the results in 
\reviseR{Table~\ref{BaselineTime}} and discussions in \reviseR{Section~\ref{sec:exp-cleanquality}}. 

\ni
5. We added errors by swapping the values across attributes and from the same 
active domain. Please refer to \reviseR{Section~\ref{sec:exp-error-analysis} -- Complex errors.}

\ni
6. \rahaBaran performs not well on \soccer because the number of generated 
features is much larger than the number of labels and thus the ML model overfits.

\ni
7. We added more detailed system settings in \reviseR{Section~\ref{sec:exp-setup}}.
\vs

\ni
{\em
{\bf [O3], [M5]}
Typographical, grammatical, and formatting errors. 
}

\ni
{\bf [A]}
Fixed in this revision. 
% Thank you for reminding us of these typos and grammatical errors, we have tried our best to eliminate them in this revision.

\vs

\ni
{\em
{\bf [M1]}
Parameter setting.
}

\ni
{\bf [A]}
We empirically set $\lambda = 0.25$, $\beta = 2$, and $\tau = 0.75$. 
We conducted an experiment on parameter tuning and reported it in the 
extended version~\cite{extended-version} due to the page limitation. 
\vs

\ni
{\em
{\bf [M2]}
Denial constraints.
}

\ni
{\bf [A]}
The UCs in \bclean covers DC. Nonetheless, we only use min/max 
constraints for numerical values, not NULL, regular expressions 
in the experiments (as described in \reviseR{Section~\ref{sec:preliminaries}}). 
In \bclean, the integrity check is automatically done by Bayesian 
inference. 
\vs

\ni
{\em
{\bf [M3]}
FD-like patterns.
}

\ni
{\bf [A]}
FDs are automatically discovered by graphical lasso (\reviseR{Section \ref{sec:network}}) 
and they are only used to generate the initial BN. We also relax it 
with similarity predicates to allow a certain degree of violation.
\vs

\ni
{\em
{\bf [M4]}
Compensative scoring model.
}

\ni
{\bf [A]}
We revised \reviseR{Section \ref{sec:intro}} to briefly introduced it.
%\vs

% \ni
% {\em
% {\bf [M5]}
% Boldface for \bclean's results.
% }

% \ni
% {\bf [A]}
% Fixed in this revision. 
% Thank you for pointing out this mistake, we have fixed it in this revision.

% \vspace{1.8ex}
% Many thanks for your support and comments!

 \newpage
 \nobalance


==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.

==> temp.tex <==
\subsubsection{Impact Of Incomplete Users' Constraint}
We produce an experiment of pruning BN with user interaction. Results show that there is no difference between before and after modification on Hospital and Soccers.After user adjustment, Hospital add edge ${state \xrightarrow state\_avg}$ and cause one more cell cleaned, while Soccers does not pose any changes. However, as for Flights, BN structure obtained by greedy search or FD-base method is obviously wrong, and the cleaning results are only 0.217precision and 0.374 recall. After adjustment by the user, the results in \ref{BaselineResult} (0.852 precision and 0.816recall) can be obtained with less than 5 minutes cost to adjust.

==> vldbblock.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%

==> vldbinfo.tex <==
%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbdoi{XX.XX/XXX.XX}
\newcommand\vldbpages{XXX-XXX}
% issue-specific
\newcommand\vldbvolume{14}
\newcommand\vldbissue{1}
\newcommand\vldbyear{2020}
% should be fine as it is
\newcommand\vldbauthors{\authors}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{URL_TO_YOUR_ARTIFACTS}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{plain} 
